Aerial Manipulation Using a Novel Unmanned Aerial Vehicle Cyber-Physical System

Unmanned Aerial Vehicles(UAVs) are attaining more and more maneuverability and sensory ability as a promising teleoperation platform for intelligent interaction with the environments. This work presents a novel 5-degree-of-freedom (DoF) unmanned aerial vehicle (UAV) cyber-physical system for aerial manipulation. This UAV's body is capable of exerting powerful propulsion force in the longitudinal direction, decoupling the translational dynamics and the rotational dynamics on the longitudinal plane. A high-level impedance control law is proposed to drive the vehicle for trajectory tracking and interaction with the environments. In addition, a vision-based real-time target identification and tracking method integrating a YOLO v3 real-time object detector with feature tracking, and morphological operations is proposed to be implemented onboard the vehicle with support of model compression techniques to eliminate latency caused by video wireless transmission and heavy computation burden on traditional teleoperation platforms.

==> doc/cfp.tex <==

% \NewsTitle{Newsletter of Technical Committee on Cyber-Physical Systems \\(IEEE Systems Council)}

% The newsletter of Technical Committee on Cyber-Physical Systems (TC-CPS) aims to provide timely updates on technologies, 
% educations and opportunities in the field of cyber-physical systems (CPS).
% The letter will be published twice a year: one issue in February and the other issue in October.
% We are soliciting contributions to the newsletter. Topics of interest include (but are not limited to):

% \begin{itemize}
%     \item Embedded system design for CPS
%     \item Real-time system design and scheduling for CPS
%     \item Distributed computing and control for CPS
%     \item Resilient and robust system design for CPS
%     \item Security issues for CPS
%     \item Formal methods for modeling and verification of CPS
%     %\item Emerging applications, e.g.~automotive system, smart energy system, internet of things, biomedical device, etc.
%     \item Emerging applications, e.g.~automotive system, smart energy system, biomedical device, etc.
% \end{itemize}

% Please directly contact the editors and/or associate editors by email to submit your contributions.

% \subsection*{Submission Deadline:}

% All contributions must be submitted by \textbf{July.~1st, 2021} in order to be included in the August issue of the newsletter.

% \vspace{.6in}
% \subsection*{Editor:}
% \begin{itemize}
%     %\item Xin Li, Carnegie Mellon University, USA, \href{mailto:xinli@cmu.edu}{xinli@cmu.edu}
%     %\item Helen Li, Duke University, USA, \href{mailto:hai.li@duke.edu}{hai.li@duke.edu}
%     \item Bei Yu, Chinese University of Hong Kong, Hong Kong \normalsize\texttt{\href{mailto:byu@cse.cuhk.edu.hk}{byu@cse.cuhk.edu.hk}}
% \end{itemize}

% \subsection*{Associate Editors:}

% \begin{itemize}
%     \item Xianghui Cao, Southeast University, China                    \normalsize\texttt{\href{mailto:xhcao@seu.edu.cn}{xhcao@seu.edu.cn}}
%     \item Long Chen, Sun Yat-Sen University, China                     \normalsize\texttt{\href{mailto:chenl46@mail.sysu.edu.cn}{chenl46@mail.sysu.edu.cn}}
%     \item Caiwen Ding, University of Connecticut, USA                  \normalsize\texttt{\href{mailto:caiwen.ding@uconn.edu}{caiwen.ding@uconn.edu}}
%     \item Keke Huang, Central South University                         \normalsize\texttt{\href{mailto:huangkeke@csu.edu.cn}{huangkeke@csu.edu.cn}}
%     \item Yier Jin, University of Florida, USA                         \normalsize\texttt{\href{mailto:yier.jin@ece.ufl.edu}{yier.jin@ece.ufl.edu}}
%     \item Subham Sahoo, Aalborg University, Denmark                    \normalsize\texttt{\href{mailto:sssa@et.aau.dk}{sssa@et.aau.dk}}
%     \item Muhammad Shafique, Vienna University of Technology, Austria  \normalsize\texttt{\href{mailto:mshafique@ecs.tuwien.ac.at}{mshafique@ecs.tuwien.ac.at}}
%     \item Umamaheswara Rao Tida, North Dakota State University, USA    \normalsize\texttt{\href{mailto:umamaheswara.tida@ndsu.edu}{umamaheswara.tida@ndsu.edu}}
%     \item Xiaolin Xu, Northeastern University, USA                     \normalsize\texttt{\href{mailto:x.xu@northeastern.edu}{x.xu@northeastern.edu}}
%     \item Ming-Chang Yang, Chinese University of Hong Kong, Hong Kong  \normalsize\texttt{\href{mailto:mcyang@cse.cuhk.edu.hk}{mcyang@cse.cuhk.edu.hk}}
%     \item Junbo Zhao, Mississippi State University, USA                \normalsize\texttt{\href{mailto:junbo@ece.msstate.edu}{junbo@ece.msstate.edu}}

%     % our previous AEs are as follows:
%     %\item Wuling Huang, Chinese Academy of Science                     \normalsize\texttt{\href{mailto:wuling.huang@ia.ac.cn}{wuling.huang@ia.ac.cn}}
%     %\item Qi Zhu, University of California at Riverside, USA          \normalsize\texttt{\href{mailto:qzhu@ece.ucr.edu}{qzhu@ece.ucr.edu}
%     %\item Abhishek Murthy, Philips Lighting Research, USA              \normalsize\texttt{\href{mailto:abhishek.murthy@philips.com}{abhishek.murthy@philips.com}}
%     %\item Rajiv Ranjan, Newcastle University, United Kingdom           \normalsize\texttt{\href{mailto:raj.ranjan@ncl.ac.uk}{raj.ranjan@ncl.ac.uk}}
%     %\item Yiyu Shi, University of Notre Dame, USA                      \normalsize\texttt{\href{mailto:yshi4@nd.edu}{yshi4@nd.edu}}
% \end{itemize}


% \begin{figure}[b!]
%   \centering
%   \includegraphics[width=.78\textwidth]{society-cover}
%   \caption*{}
% \end{figure}




==> doc/cover.tex <==
% {
% \setlength{\parskip}{.2in}

% %\textbf{Editorial}

% \textbf{Technical Articles}
% \vspace{-.2in}
% \begin{itemize}
%     \item{Author 1},
%         \textit{``Title 1''}
%     \item{Author 2},
%         \textit{``Title 2''}
% \end{itemize}



% \textbf{Summary of Activities}

% \textbf{Call for Contributions}

% }


% \begin{figure}[b!]
%   \centering
%   \includegraphics[width=.38\textwidth]{logo-tccps}
%   \caption*{}
% \end{figure}



